Distributed DoS Attack Detection in SDN: Trade offs in Resource Constrained Wireless Networks

The Software-defined networking(SDN) paradigm centralizes control decisions to improve programmability and simplify network management. However, this centralization turns the network vulnerable to denial of service (DoS) attacks, and in the case of resource constrained networks, the vulnerabilities escalate. The main shortcoming in current security solutions is the trade off between detection rate and complexity. In this work, we propose a DoS attack detection algorithm for SDN resource constrained networks, based on recent results on non-parametric real-time change point detection, and lightweight enough to run on individual resource constrained devices. Our experiment results show detection rates and attacker identification probabilities equal or over 0.93.

==> related-work.tex <==
\section{Related work} \label{sec:related}

Pioneer works compare probability distributions of time series over different intervals (past and present) obtaining promising results \cite{basseville1993detection}. The main idea of these works was to set an alarm when a significant difference between two distributions is detected. Examples of methods using this strategy are: cumulative sum (CUSUM)\cite{basseville1993detection}, generalized likelihood-ratio method \cite{481608}, and change finder \cite{1599387}. 

There is another group of methods that measure the difference between subspaces to detect dissimilarity between past and present time series intervals. Two relevant approaches are \textit{subspace identification} methods, which can be interpreted as a singular value decomposition of a weighted matrix \cite{QIN20061502}, and \textit{Krislov subspace learning} based algorithms, which are convenient when working with indefinite and asymmetrical matrixes \cite{2018arXiv181109025F}. 

Change point detection algorithms have been used in several applications of different fields, as quality control \cite{cpdynamical}, industrial processes \cite{NICULITA2014115}, medical applications \cite{qi2014novel}, and security attacks detection for WSN \cite{1580418} and SDN \cite{8115796}. There are multiple proposals in the literature that use change point detection in WSN to detect anomalies. \citeonline{5541872} proposed a detection mechanism of sinkhole attacks in WSN monitoring only node's CPU usage. Their main hypothesis is that CPU usage in malicious nodes is higher than 80\%, thus, they addressed this issue as a change point detection problem. The algorithm was tested through simulations in a network with 2000 nodes, programming 5\% of them as malicious nodes, and evaluating detection time, false positive rate, and effectiveness. The whole evaluation was conducted using MATLAB. Authors claim their proposal can detect malicious nodes in a short time and with low false positive, but their results are not compared with any other proposal. Also, since the base station is who decides if a node is a malicious node, there is also the possibility that the malicious node lies when sending this information, but authors do not consider this possibility. 

\citeonline{exhausting2013} models WSN energy consumption when the networks is under an energy exhaustion attack and proposes some methods to detect it. Part of these methods is to use change point analysis to detect an intrusion by monitoring the bit error probability. The main hypothesis is that bit error probability change when the network is under attack. However, the author does not present implementation nor results about the change point detection. \citeonline{8610497} use a CUSUM-based change point detection algorithm to detect and locate jammers attackers in WSN. Their proposal was tested using simulations, varying the number of nodes (8 and 16) and the topology (square, circle and diamond). Some weak points of this paper are: i) authors do not present results about the jammers detection, only about the location error and ii) there is no information about the simulator software. \citeonline{5934944} introduces the self-diagnosis concept in WSN as a way to decentralized fault detection decisions, that are commonly taken in the sink, and encourage the sensor nodes to join this process. Authors used change point detection algorithms to decide if a node should join the fault detection process.


%For example, \citeonline{chen2007distributed} proposed a distributed DoS (DDoS) flooding attack detection for wired networks using change point analysis and Change Aggregation Tree (CAT). Each router executes a change point detection instance and alerts the CAT server in case of anomalous traffic. The CAT server decides how to proceed based on the number of alerts received. This detection mechanism was tested on the DETER testbed \cite{1649172} at USC Information Sciences Institute using more than 180 nodes.  

There are also some proposals in the literature for wired SDN using change point detection.
\citeonline{8115796} proposed a distributed DoS (DDoS) detection attack and their main objective was to provide a unique solution to detect several fundamentally different DDoS attacks in SDN. Authors use CUSUM technique and incorporate and adaptive threshold to reduce false alarms. The most important results are an average false alarm rate under 11.64\% and average detection time of 4.15 seconds. \citeonline{7368594} and \citeonline{mahrach2018sdn} propose change point detection mechanisms to detect flooding attacks. The first work used a detection scheme called ChangeFinder \cite{1599387} and the latter proposed a simple CUSUM algorithm with one threshold. \citeonline{7368594} main objective was to detect the attack before the network congestion. To address this issue, they used multiple detection servers running the ChangeFinder mechanism to reduce false alarms caused by sudden increase of traceroute packets. The detection mechanism performance was evaluated through simulations varying the network topology size but using the same number of attackers and decoy servers. Authors reported their proposal is able to detect the attack before the network congestion. Unlike \citeonline{7368594}, \citeonline{mahrach2018sdn} do not present results of their proposal.

From previous works, we noticed change point detection mechanisms are commonly used in intrusion detection for WSN and SDN. In this chapter we test a change point detection algorithm to detect DoS attacks in SDWSN. We used \citeonline{skaperas:hal-01997965} proposal to detect a change point in data packets delivery rate metric when the networks is under a FDFF and FNI attack (Chapter \ref{sec:attacks}).

==> tab-1.tex <==
\begin{table}[htb]
\caption{Detection results for FDFF attack d:100 Critical value 0.95}
\begin{tabular}{|c|c|l|l|c|c|c|}
\hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Percentage of \\ \\ Attackers\end{tabular}}} & \multicolumn{6}{c|}{\textbf{Topology size}}                                                                                           \\ \cline{2-7} 
                                                                                                & \multicolumn{3}{c|}{\textbf{36}}                                                       & \multicolumn{3}{c|}{\textbf{100}}            \\ \cline{2-7} 
                                                                                                & \textbf{Median} & \multicolumn{1}{c|}{\textbf{MAD}} & \multicolumn{1}{c|}{\textbf{DR}} & \textbf{Median} & \textbf{MAD} & \textbf{DR} \\ \hline
5                                                                                               &                 &                                   &                                  &                 &              &             \\ \hline
10                                                                                              & 254.5             & 6.5                               & 0.9                              & 239             & 13           & 0.70        \\ \hline
20                                                                                              &                 &                                   &                                  &                 &              &             \\ \hline
\end{tabular}
\end{table}


\begin{table}[htb]
\caption{Detection results for FNI attack d:100 Critical value 0.95}
\begin{tabular}{|c|c|l|l|c|c|c|}
\hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Percentage of \\ \\ Attackers\end{tabular}}} & \multicolumn{6}{c|}{\textbf{Topology size}}                                                                                           \\ \cline{2-7} 
                                                                                                & \multicolumn{3}{c|}{\textbf{36}}                                                       & \multicolumn{3}{c|}{\textbf{100}}            \\ \cline{2-7} 
                                                                                                & \textbf{Median} & \multicolumn{1}{c|}{\textbf{MAD}} & \multicolumn{1}{c|}{\textbf{DR}} & \textbf{Median} & \textbf{MAD} & \textbf{DR} \\ \hline
5                                                                                               &                 &                                   &                                  &                 &              &             \\ \hline
10                                                                                              & 235.5           & 3.5                               & 1                                & 236             & 5.5          & 1           \\ \hline
20                                                                                              &                 &                                   &                                  &                 &              &             \\ \hline
\end{tabular}
\end{table}

==> tab-parameters.tex <==
\begin{table}[htb]
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
% \todo{adicionar novos cenários (adicionado tipos de flow setup e P2P-RPL nos MOPs)} 
% \todo{olhar tabela II de \cite{sdnwise-testbed} e ver o que eles colocaram como referência}
\caption{Simulation Parameters}
\label{tab:parameters}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll}
\hline
\multicolumn{2}{|l|}{\textbf{Simulation parameters}}                                                                         \\ \hline
\multicolumn{1}{|l|}{Topology}                          & \multicolumn{1}{l|}{Square grid}                          \\ \hline
\multicolumn{1}{|l|}{Number of nodes}                   & \multicolumn{1}{l|}{36 and 100}     
\\ \hline
\multicolumn{1}{|l|}{Simulation duration}                & \multicolumn{1}{l|}{36000 s}     
\\ \hline
\multicolumn{1}{|l|}{Node boot interval}                & \multicolumn{1}{l|}{$[0, 1]$ s}                           \\ \hline
\multicolumn{1}{|l|}{Number of sinks}                   & \multicolumn{1}{l|}{2}                                 \\ \hline
\multicolumn{1}{|l|}{Sinks position}                    & \multicolumn{1}{l|}{Middle of the grid edge}              \\ \hline
\multicolumn{1}{|l|}{Data traffic rate}                 & \multicolumn{1}{l|}{1 packet every 30 seconds}            \\ \hline
\multicolumn{1}{|l|}{Management traffic rate}           & \multicolumn{1}{l|}{1 packet every two minutes}            \\ \hline
\multicolumn{1}{|l|}{Data payload size}                 & \multicolumn{1}{l|}{10 bytes}                             \\ \hline
\multicolumn{1}{|l|}{Management payload size}           & \multicolumn{1}{l|}{10 bytes}                       \\ \hline
\multicolumn{1}{|l|}{Data traffic start time}           & \multicolumn{1}{l|}{$[2, 3]$ min}                         \\ \hline
\multicolumn{1}{|l|}{Radio module power}                & \multicolumn{1}{l|}{0 dB}                         \\ \hline
\multicolumn{1}{|l|}{Distance between neighbors}        & \multicolumn{1}{l|}{50 m}                         \\ \hline
\multicolumn{1}{|l|}{Attacks begins after}                  & \multicolumn{1}{l|}{28800 s}                         \\ \hline


\\ \hline
\multicolumn{2}{|l|}{\textbf{IT-SDN parameters}}                                                                             \\ \hline
\multicolumn{1}{|l|}{Controller position}               & \multicolumn{1}{l|}{center}                               \\ \hline
% \multicolumn{1}{|l|}{Controller retransmission timeout} & \multicolumn{1}{l|}{60 s}                                 \\ \hline
\multicolumn{1}{|l|}{ND protocol}                       & \multicolumn{1}{l|}{Collect-based}                        \\ \hline
\multicolumn{1}{|l|}{Link metric}                       & \multicolumn{1}{l|}{ETX}                                  \\ \hline
% \multicolumn{1}{|l|}{Neighbor report max frequency}     & \multicolumn{1}{l|}{1 packer per minute}                  \\ \hline
\multicolumn{1}{|l|}{CD protocol}                       & \multicolumn{1}{l|}{none}                                 \\ \hline
\multicolumn{1}{|l|}{Flow setup}                        & \multicolumn{1}{l|}{source routed}                        \\ \hline
\multicolumn{1}{|l|}{Route calculation algorithm}       & \multicolumn{1}{l|}{Dijkstra}                             \\ \hline
\multicolumn{1}{|l|}{Route recalculation threshold}     & \multicolumn{1}{l|}{$10\%$}                               \\ \hline
\multicolumn{1}{|l|}{{Flow setup types}}     & \multicolumn{1}{l|}{{regular or source routed}}                               \\ \hline
\multicolumn{1}{|l|}{{Flow table size}}     & \multicolumn{1}{l|}{{10 entries}}                               \\ \hline
\end{tabular}
}

\end{table}
